NPGLM: A Non-Parametric Method for Temporal Link Prediction

In this paper, we try to solve the problem of temporal link prediction in information networks. This implies predicting the time it takes for a link to appear in the future, given its features that have been extracted at the current network snapshot. To this end, we introduce a probabilistic non-parametric approach, called "Non-Parametric Generalized Linear Model" (NP-GLM), which infers the hidden underlying probability distribution of the link advent time given its features. We then present a learning algorithm for NP-GLM and an inference method to answer time-related queries. Extensive experiments conducted on both synthetic data and real-world Sina Weibo social network demonstrate the effectiveness of NP-GLM in solving temporal link prediction problem vis-a-vis competitive baselines.

==> acknowledge.tex <==
\section*{Acknowledgements}
We would like to thank anonymous reviewers for their comments and feedbacks on this paper. We also appreciate ICT Innovation Center of Sharif University of Technology for their financial support.
